Federated Learning with Manifold Regularization and Normalized Update Reaggregation

Federated Learning (FL) is an emerging collaborative machine learning framework where multiple clients train the global model without sharing their own datasets. In FL, the model inconsistency caused by the local data heterogeneity across clients results in the near-orthogonality of client updates, which leads to the global update norm reduction and slows down the convergence. Most previous works focus on eliminating the difference of parameters (or gradients) between the local and global models, which may fail to reflect the model inconsistency due to the complex structure of the machine learning model and the Euclidean space's limitation in meaningful geometric representations. In this paper, we propose FedMRUR by adopting the manifold model fusion scheme and a new global optimizer to alleviate the negative impacts. Concretely, FedMRUR adopts a hyperbolic graph manifold regularizer enforcing the representations of the data in the local and global models are close to each other in a low-dimensional subspace. Because the machine learning model has the graph structure, the distance in hyperbolic space can reflect the model bias better than the Euclidean distance. In this way, FedMRUR exploits the manifold structures of the representations to significantly reduce the model inconsistency. FedMRUR also aggregates the client updates norms as the global update norm, which can appropriately enlarge each client's contribution to the global update, thereby mitigating the norm reduction introduced by the near-orthogonality of client updates. Furthermore, we theoretically prove that our algorithm can achieve a linear speedup property for non-convex setting under partial client participation.Experiments demonstrate that FedMRUR can achieve a new state-of-the-art (SOTA) accuracy with less communication.

==> method.tex <==
\section{Algorithm}
\label{alo-a}


\begin{algorithm}
  \caption{Client-Momentum-LPF (server)}\label{algo-s}
  \begin{algorithmic}
    \STATE \textbf{Input:}  {initial parameter $w^{0}$; momentum coefficient $\alpha$; perturbation (filter) radius $\gamma$;} \\
    {local interval $K$ ; communication rounds $T$; set of selected clients $S_t$; local learning rate $\eta_l$.} 
    \STATE \textbf{Output:} {Global parameter $w^{t}, \forall i \in T$.}
    \STATE \textbf{Initialization:} {Initialize $\triangle^0=0$ and $w^{0}$ as the global parameter at the server.}
    \STATE {For $t=0,1,...,T-1$ do:}
    \STATE {\quad The server compute the covariance matrix $\sum = \text{diag} ({\lVert w_l^{t} \rVert}_{l=1}^{L})$.}
    \STATE {\quad The server selected $\lvert S_t \rvert$ clients from all clients.}
    \STATE {\quad The server broadcasts parameter $w^t$, global update $\triangle^t$ and covariance matrix $\sum$ to $S_t$.}
    \STATE {\quad For client $ i \in S_t$ in parallel do:}
    \STATE {\quad \quad Set $w_i^{t,0} \leftarrow w^t + \mathcal{N}(0, \gamma\sum)$.}
    \STATE {\quad \quad Use Algorithm \ref{algo-l} $(w_i^{t,0}, \eta_l, K, \alpha, \triangle^t, \gamma)$ to get $\triangle_i^t$ and communicate it to the server.}
    \STATE {\quad End for}
    \STATE {\quad Compute $\triangle^{t+1} = \frac{1}{\lvert S_t \rvert} \sum_{i \in S_t} \triangle_i^t$.}
    \STATE {\quad Update global parameter $w^{t+1} = w^t - \eta_g \triangle^{t+1}$.}
    \STATE {End for.}
  \end{algorithmic}
\end{algorithm}


\begin{algorithm}
  \caption{Client-Momentum-LPF (client)}\label{algo-l}
  \begin{algorithmic}
    \STATE \textbf{Input:} {local parameter $w_i^{t,0}$; local learning rate $eta_l$; local interval $K$;} \\
    {momentum coefficient $\alpha$; global update (last round)$\triangle^t$; perturbation (filter) radius $\gamma$.}
    \STATE \textbf{Output:} {local update $\triangle_i^t$.}
    \STATE {For $k=0 ,..., K-1$ do:}
    \STATE {\quad Compute $v_i^{t,k+1} = \alpha \nabla F_i(w_i^{t,k}) + (1-\alpha) \triangle^t$.}
    \STATE {\quad Update $w_i^{t,k+1} = w_{i}^{t,k} - \eta_l v_i^{t,k+1}$.}
    \STATE {End for.}
    \STATE {$\triangle_i^t = w_i^{t,K} - w_i^{t,0}$.}
  \end{algorithmic}
\end{algorithm}
